On Catalan Constant Continued Fractions

The Ramanujan Machine project detects new expressions related to constants of interest, such as $\zeta$ function values, $\gamma$ and algebraic numbers (to name a few). In particular the project lists a number of conjectures concerning the Catalan constant $G= 0.91596559\ldots$ We show how to generate infinitely many. We used an ad hoc software toolchain and rather tedious mathematical developments. Because we do not provide a proper peer-reviewed proof of the relations given here we do not claim them to be theorems.

==> students.tex <==
\section{The Challenge}

Several people asked us more information on the concrete work that remains to be done on this question. Hence we edited this note to explain exactly what is the question.

We have a code that given $\kappa$ and $c$ outputs, using lattice reduction the constants $\alpha_{c,\kappa}$, $\beta_{c,\kappa}$ and $\gamma_{c,\kappa}$. We generated those constants for $1\leq \kappa\leq 15$ and $1\leq c \leq 40$ (we can easily go beyond those bounds if needed).

Now, we know what is the ratio $\rho_{c,\kappa}=\frac{\alpha_{c,\kappa}}{\gamma_{c,\kappa}}$ as we have a formula for it. For now just leave $\beta_{c,\kappa}$ aside. The challenge consists in using your imagination and any algorithmic tools to reverse-engineer what $\alpha_{c,\kappa}$ and  $\gamma_{c,\kappa}$ are -- given (1) the unlimited number of examples that we have and can generate (2) the ratio of those quantities that we know and (3) the formulae for the cases $0\leq\kappa\leq 2$.

When we generate those constants and factor them we stumble on many very small factors. Clearly $\alpha_{c,\kappa}$ and  $\gamma_{c,\kappa}$ are formed of products of factor-rich integers generated by functions such as $x!$, $x!!$, $C_x$, $\binom{x}{y}$, $2^x$ etc. Certainly with offsets, e.g. $(ax+b)!$, $2^{ax+b}$ etc.

The challenge consists in using your imagination and insight to identify what is in $\alpha_{c,\kappa}$ and  $\gamma_{c,\kappa}$ departing from the data file we provide and the hint given by the known ratio $\rho_{c,\kappa}$ as well as the explicit examples we know for $\kappa=1$ and $\kappa=2$ (we recommend to put $\kappa=0$ aside as it does not seem to fit the general scheme).

For now do not bother about $\beta_{c,\kappa}$ as it obeys another logic and once we have $\alpha_{c,\kappa}$ and  $\gamma_{c,\kappa}$ we could start to look into $\beta_{c,\kappa}$ using other techniques.

In the data files, the constants appear in the following order: 

$$\{c,\kappa,\rho_{c,\kappa},\alpha_{c,\kappa},\gamma_{c,\kappa}\}$$

The second data file contains the same data but gives $\alpha_{c,\kappa},\gamma_{c,\kappa}$ already factored so can visualize what is in them.

This will give a \textcolor{red}{very nice} general conjecture.

For those curious about the next step after we conquer $\alpha_{c,\kappa}$ and  $\gamma_{c,\kappa}$: $\beta_{c,\kappa}$ is a second order recursion with polynomial coefficients. Once we have $\alpha_{c,\kappa}$ and  $\gamma_{c,\kappa}$ the plan is to solve for the values of $\beta_{c,\kappa}$ and interpolate the values of the coefficients governing the generation of $\beta_{c,\kappa}$. Then we will use again our imagination and inspiration to look for regularities in those polynomials but in any case, we will have a procedure to generate them (the interpolation) for any given $c,\kappa$. This would be a great progress.
